Multimodal Misinformation Detection using Large Vision-Language Models

The increasing proliferation of misinformation and its alarming impact have motivated both industry and academia to develop approaches for misinformation detection and fact checking. Recent advances on large language models (LLMs) have shown remarkable performance in various tasks, but whether and how LLMs could help with misinformation detection remains relatively underexplored. Most of existing state-of-the-art approaches either do not consider evidence and solely focus on claim related features or assume the evidence to be provided. Few approaches consider evidence retrieval as part of the misinformation detection but rely on fine-tuning models. In this paper, we investigate the potential of LLMs for misinformation detection in a zero-shot setting. We incorporate an evidence retrieval component into the process as it is crucial to gather pertinent information from various sources to detect the veracity of claims. To this end, we propose a novel re-ranking approach for multimodal evidence retrieval using both LLMs and large vision-language models (LVLM). The retrieved evidence samples (images and texts) serve as the input for an LVLM-based approach for multimodal fact verification (LVLM4FV). To enable a fair evaluation, we address the issue of incomplete ground truth for evidence samples in an existing evidence retrieval dataset by annotating a more complete set of evidence samples for both image and text retrieval. Our experimental results on two datasets demonstrate the superiority of the proposed approach in both evidence retrieval and fact verification tasks and also better generalization capability across dataset compared to the supervised baseline.

==> Tables/fakenews_detection_Factify.tex <==
\begin{table*}[t]
%\small
\centering
\setlength{\tabcolsep}{9pt}
\caption{Precision(P), Recall (R) and F-score(F1) of models for fake news detection task on ّ Factify validation set. Mistral-Open-Orca model is used for text evidence and LLaVA model is used for multimodal evidence. All results are with K=2}
\label{table:fndetection_factify}
\begin{tabular}{lcccccccccc}
\toprule
\multirow{2}{*}{\bf{Method}} & \multirow{2}{*}{\bf{Evidence}} & \multirow{2}{*}{\bf{Modality}} & \multicolumn{3}{c}{\bf{Real}} & \multicolumn{3}{c}{\bf{Fake}} &  \multirow{2}{*}{\bf{Acc}}  & 
 \multirow{2}{*}{\bf{F1}}\\\cmidrule(lr){4-6} \cmidrule(lr){7-9} & & & \bf{$P$} & \bf{$R$} & \bf{$F1$} & \bf{$P$} & \bf{$R$} &\bf{$F1$}\\
\midrule
\multirow{2}{*}{\bf{\FNmodelName}} & Retrieved & text & 0.968 & 0.494 & 0.654  & 0.488 & 0.967 & 0.649  & 0.652 & 0.651 \\ & Gold & text & 0.948 & 0.591 & 0.728 & 0.533 & 0.935 & 0.679 & 0.706 & 0.703\\
\midrule
\multirow{2}{*}{\bf{\FNmodelName}} & Retrieved & multimodal &  &  &   &  &  &   &  &  \\ & Gold & multimodal & 0.974 & 0.465 & 0.629 & 0.477 & 0.975 & 0.640 & 0.635 & 0.635\\
\midrule
\bf{MOCHEG} & Gold & multimodal & 0.740 & 0.588 &  0.655 & 0.516 &  0.670 &  0.584 & 0.612 & 0.619 \\

\bottomrule
\end{tabular}
\end{table*}

==> Tables/fakenews_detection_Mocheg.tex <==
\begin{table*}[t]
%\small
\centering
\setlength{\tabcolsep}{9pt}
\caption{Precision(P), Recall (R) and F-score(F1) of models for fake news detection task on MOCHEG test set. Mistral-Open-Orca model is used for text evidence and InstructBlip model is used for multimodal evidence. All results are with K=5}
\label{table:fndetection}
\begin{tabular}{lcccccccccc}
\toprule
\multirow{2}{*}{\bf{Method}} & \multirow{2}{*}{\bf{Evidence}} & \multirow{2}{*}{\bf{Modality}} & \multicolumn{3}{c}{\bf{Real}} & \multicolumn{3}{c}{\bf{Fake}} &  \multirow{2}{*}{\bf{Acc}}  & 
 \multirow{2}{*}{\bf{F1}}\\\cmidrule(lr){4-6} \cmidrule(lr){7-9} & & & \bf{$P$} & \bf{$R$} & \bf{$F1$} & \bf{$P$} & \bf{$R$} &\bf{$F1$}\\
\midrule
\multirow{2}{*}{\bf{\FNmodelName}} & Retrieved & text & 0.659 & 0.826 &  0.733 & 0.767 & 0.574 &  0.656 & 0.700 &  \bf{0.695}\\ & Gold & text & 0.870 & 0.482 & 0.621 & 0.642 & 0.928 & 0.759 & \bf{0.705} & 0.690\\
\midrule
\multirow{2}{*}{\bf{\FNmodelName}} & Retrieved & text+image & 0.661 & 0.688 &  0.675 & 0.544 & 0.513 &  0.528 & 0.615 &  0.601\\ & Gold & text+image & 0.708 & 0.712 & 0.710 & 0.600 & 0.595 & 0.597 & 0.663 & 0.654\\
\midrule
\bf{MOCHEG} & Gold & text+image & 0.858 & 0.353 &  0.501 & 0.638 & 0.845 &  0.727 & 0.599 &  0.614\\

\bottomrule
\end{tabular}
\end{table*}

==> Tables/prompts_table.tex <==
\begin{table*}[t] % Use table* to span both columns
\centering
\begin{minipage}[t]{0.30\textwidth} % Adjust width as needed
\centering
\caption{Results of \modelName for both text and image retrieval with different prompts.}
\label{tab:prompts_resutls}
\begin{tabular}{cccccc}
\toprule
\bf{Modality} & \bf{Prompts} & \bf{K} & \bf{Pre} & \bf{Rec} & \bf{mAP}\\
\midrule
\multirow{3}{*}{\bf{text}} & \multirow{3}{*}{\bf{A}} & 1 & 26.19 & 7.59 &  26.19 \\ & &  5 & 14.62 &  18.31 & 15.82 \\  & & 10 & 10.81 & 24.60 & 15.40 \\
\midrule
\multirow{3}{*}{\bf{text}} & \multirow{3}{*}{\bf{B}} & 1 & 19.94 & 5.32 &  19.94 \\ & &  5 & 10.81 &  13.09 & 11.23 \\  & & 10 & 7.71 & 17.91 & 10.78 \\
\midrule
\multirow{3}{*}{\bf{text}} & \multirow{3}{*}{\bf{C}} & 1 & 21.39 & 5.83 &  21.39 \\ & &  5 & 17.84 &  9.22 & 16.08 \\  & & 10 & 7.91 & 17.95 & 11.58 \\
\midrule
\multirow{3}{*}{\bf{image}} & \multirow{3}{*}{\bf{D}} & 1 & 7.71 & 5.36 &  7.18 \\ & &  5 & 3.66 &  13.27 & 8.54 \\  & & 10 & 2.54 & 17.92 & 9.22 \\
\midrule
\multirow{3}{*}{\bf{image}} & \multirow{3}{*}{\bf{E}} & 1 & 6.89 & 5.20 &  6.89 \\ & &  5 & 3.73 &  13.47 & 8.46 \\  & & 10 & 2.59 & 18.90 & 9.26 \\
\midrule
\multirow{3}{*}{\bf{image}} & \multirow{3}{*}{\bf{F}} & 1 & 9.65 & 7.13 &  9.65 \\ & &  5 & 4.19 &  14.80 & 10.42 \\  & & 10 & 2.54 & 18.16 & 10.96 \\
\bottomrule
\end{tabular}
\end{minipage}
\hfill % Fill horizontal space between minipages
\begin{minipage}[t]{0.45\textwidth} % Adjust width as needed
\centering
\begin{tabular}{cp{7.5cm}}
\toprule
\bf{Abb} & \bf{Prompt}\\
\midrule
A & Is this corpus related to the query? Answer with yes or no.\\
B &  Is this query and corpus mentioning the same person or topic? Answer with yes or no.\\
C & Is this corpus an evidence for the query? answer with yes or no.\\
D & Does this query describes the image?\\
E & Based on the query below, is it related to the image?\\
F & Is this image and text query mentioning the same person or topic?\\
\bottomrule
\end{tabular}
\caption{Details of each text prompts with its abbreviation(Abb)}
\label{tab:prompts_details}
\end{minipage}
\end{table*}

==> sections/Methodology.tex <==

In this section, we propose an  LLM-involved pipeline for multimodal fake news detection to predict whether a post is \textit{fake}~($y=0$) or \textit{real}~($y=1$). As illustrated in Figure~\ref{fig1}, it consists of two main components: (1)~An evidence retrieval component which gets a claim and a large collection of web sources including articles and images as input and automatically retrieve information sources which are relevant to the claim. (2)~ A fake news detection component which predicts whether the claim is fake or real based on the retrieved evidences.
\subsection{Evidence Retrieval}
To solve this task, we apply two existing large language models to retrieve text and image evidence separately and provide Large Language Models for Evidence Retrieval~(LLM4EV). For both subtasks we use (V)LLms as  ranker which aims to rerank a set of evidences that are retrieved by first-stage retrieval model. Unlike existing supervised ranking methods which suffer from  weak generalizability to new domains, and restricted commercial  use~\cite{DBLP:journals/corr/abs-2112-09118}, the goal is to utilize the excellent ability of LLMs on zero-shot learning to improve evidence retrieval.
\subsubsection{Text Retrieval} The bottom left in Figure~\ref{fig1} illustrates the approach for text evidence retrieval. Given an input claim~$({Q}_{i})$ and a document corpus~$(C)$, we first apply~\cite{DBLP:mocheg} as the first stage retriever to get top-N most related documents. Then, we employ Mistral model~\cite{DBLP:Mistral} and input each ~$(\mathbf{Q}_{i}, \mathbf{C}_{j}),\ j \in {\{1,N}\}$ with a prompt template for relevance generation. Mistral model is instructed to output “Yes” if the query and corpus are relevant or “No” if they are irrelevant. We use the log probability of the model to extract the scores for all pairs in order to rank them. The relevance score~$({S}_{ij})$ is measured by the probability of model generating the word ‘Yes’ or ‘No’ :
\begin{equation}
{S}_{ij} = 
\begin{cases}
    \lambda * P_{j}(Yes) & \text{if output Yes} \\
    \lambda * (1-P_{j}(Yes)) & \text{if output No}
\end{cases}
\end{equation}
where $\lambda=1$ if output is Yes and $10^{-4}$ if output is No. For each query, we further rank all the candidate evidence~$({C}_{j})$ based on~${S}_{ij}$ and select the top-K as the text evidence. 
\subsubsection{Image Retrieval} The top left in Figure 2 illustrates the
approach for image evidence retrieval. Given an input claim~$({Q}_{i})$ and the image corpus~$(C)$, same as text retrieval, we first use the same first stage retriever to get the top-N most related images. Here, we employ InstructBLIP~\cite{DBLP:Instruct-blip} model and construct the prompt template for relevancy generation. To extract relevancy scores of~${S}_{ij}$, we use CLIP~\cite{DBLP:CLIP} similarity scores:\begin{equation}
{S}_{ij} = 
\begin{cases}
    1 * S(C_{j}) & \text{if output Yes} \\
    10^{-4} * S(C_{j}) & \text{if output No}
\end{cases}
\end{equation}
where $S(C_{j})$ is the cosine similarity between CLIP representation of the claim and candidate image evidence~$C_{j}$. Then, we rank all the candidate evidence~$({C}_{j})$ based on~${S}_{ij}$
and select the top-K as the image evidence.
\subsubsection{Label Inconsistency}
\label{sec:label_inconsistency}
Mocheg~\cite{DBLP:mocheg} is one the pioneering datasets for multimodal evidence retrieval which provides a valuable resource for training and evaluating multimodal retrieval models. However, a significant challenge arises from label inconsistency. For example in image retrieval, each claim is associated with a set of labeled images meant to serve as ground truth image evidence, while there exist other visually similar images within the dataset that are left unlabeled~(Figure\ref{fig3}). This is also the case for text retrieval. This inconsistency undermines the integrity of the dataset  introduces ambiguity and noise into the learning process and leads to diminished performance in identifying relevant evidence.

To address label inconsistency in multimodal evidence retrieval and ensure fair and accurate assessments of system performance, we annotate a clean subset of Mocheg test set for both text and image evidence retrieval. For each modality, we annotate three sets:~(1) Mocheg-top10,~(2) LLM4IR-top10 and (3) Union. Figure~\ref{fig4} demonstrates an example of the annotation.
\paragraph{Mocheg-top10} We apply Mocheg method to retrieve top-10 most related text and image evidence separately for all claims within the test set. Subsequently, expert annotate top 10 retrieved evidence for randomly selected 10 claims. The annotation process is on three levels~(1) Entity-level: this denotes when the candidate evidence is relevant but solely shares the same entity or topic without offering direct support or refutation of the claims.~(2) Evidence-level: when the candidate evidence provides direct evidence to support or reject the claim.~(3) total: if either of the preceding two levels is deemed true, we designate the total relevancy as true.
\paragraph{LLM4IR-top10} For this set, we employ LLM4IR model to retrieve top 10 most related text and image evidences for all claims in the test set. The annotation process is just like previous set mentioned above. Note that we used the same claim ids which we sampled in the above set.
\paragraph{Union} We combine Mocheg-top10 and LLM4IR-top10 sets to form the union. In cases where there is overlap for a claim, we retain only the distinct candidate evidence. The idea is to ensure all the top 10 relevant candidate evidences are labeled for the sampled claims by considering both baselines.
\subsection{Fake News Detection}
Based on the retrieved text and image evidence, we further design a fake news detection component to predict the veracity of each input claim, which is shown in the right of figure~\ref{fig2}. To this end, we consider two models, a Mistral model based on text evidence and an InstructBLIP model based on multimodal evidence. We then pair each piece of evidence with the input claim and create the model template. Models are instructed to answer 'Yes' if the evidence confirms the claim and 'No' if it rejects it. We have used prompt based classification for 'Yes' and 'No' tokens to ensure the model output is robust and we avoid hallucination. Softmax function is used to normalize

